A Robinson-Schensted Correspondence for Partial Permutations

We study the Steinberg variety associated to matrix Schubert varieties, and develop a Robinson-Schensted type correspondence, $\tau\leftrightarrow(\Lambda,\mathsf Q,\mathsf P)$. Here $\tau$ is a partial permutation of size $p\times q$, $\Lambda$ an admissible signed Young diagram of size $p+q$, and $\mathsf P$ (resp. $\mathsf Q$) a standard Young tableau of size $p$ (resp. $q$) whose shape is determined by $\Lambda$. By embedding the matrix Schubert variety into a Schubert variety, we find a close relationship between the combinatorics of the classical Robinson-Schensted-Knuth correspondence and our bijection. We also show that an involution $(\Lambda,\mathsf Q,\mathsf P)\mapsto(\Lambda^\vee,\mathsf P,\mathsf Q)$ corresponds to projective duality on matrix Schubert varieties.

==> old.tex <==
\begin{framed}
\subsection{Signed Young Diagrams}
\label{syd}
Consider $(x,y)\in\mathcal O_\Lambda$, for some signed Young diagram $\Lambda$. 
The diagram $\Lambda$ can be recovered from the sequence of tuples \begin{align*}
	\left(\rk(xy)^i,\rk(yx)^i,\rk (yx)^iy,\rk(xy)^ix\right)_{i\geq 0}.
\end{align*}
Now, $\rk(xy)^i$ (resp. $\rk(yx)^i$) can be recovered from $sh(xy)$ (resp. $sh(yx)$).

Next, it follows from\begin{align*}
	\begin{pmatrix} -yx			&0	\\ x		&0	\end{pmatrix}^{i+1}=
	\begin{pmatrix} (-yx)^{i+1}	&0	\\ (-xy)^ix	&0	\end{pmatrix}
\end{align*}
that the sequence $\rk (xy)^ix$ can be deduced from the Jordan type of $\begin{pmatrix} -yx&0\\x&0\end{pmatrix}$.
Similarly, the sequence $\rk (yx)^iy$ can be deduced from the Jordan type of $\begin{pmatrix} -yx&y\\0&0\end{pmatrix}$.
\end{framed}

\begin{problem}
Given a signed Young diagram $\Lambda$, characterize the $\tau$ such that a generic point of $Z_\tau$ maps to $\mathcal O_\Lambda$ under $\widetilde\mu$.
\end{problem}

\subsection{Partial Permutations}
\label{partialTow}
Let $B_H$ be the upper triangular Borel subgroup in $H$, and let $Mat_n$ be the set of $n\times n$ matrices.
The embedding $f:Mat_n\hookrightarrow G$, given by \[
	x\mapsto\begin{pmatrix}	1&0	\\ x&1\end{pmatrix},
\]
induces a bijection $B_H\backslash M/B_H\cong P\backslash G/Q=\nicefrac{\left(\nicefrac GP\times\nicefrac GQ\right)}G$, which we describe below.

The points of $B_H\backslash M/B_H$ are indexed by partial permutation matrices $\tau$ of size $n\times n$.
We index the $G$-orbits of $\nicefrac{\left(\nicefrac GP\times\nicefrac GQ\right)}G$ by their $w$-matrices, see \cref{rankMatrix}.
%the $w\in S_N$ which are \emph{maximal} for the left action of $W_P$ and the right action of $W_Q$.

Consider a partial permutation $\tau$, and let $r=rk(\tau)$. 
The corresponding rank matrix $w_\tau$ is given by, 
\begin{align*}
	\begin{pmatrix}
		A	& r\\	
		\tau& B
	\end{pmatrix}.
\end{align*}
Here $A$ (resp. $B$) is a $1\times n$ (resp. $n\times 1$) matrix with $1$ in the $i^{th}$ column (resp. row) if and only if $\tau$ has no non-zero entry in the $i^{th}$ column (resp. row).

%Here $J_r$ is the $r\times r$ matrix with $1$s on the anti-diagonal, and $0$ elsewhere.
%The matrix $A$ (resp. $B$) is of size $n-r\times n$ (resp. $n\times n-r$). 
%Each row (resp. column) of $A$ (resp. $B$) has a unique non-zero entry (equal to $1$). 
%A column (resp. row) of $A$ (resp. $B$) has a non-zero entry (equal to $1$) if and only if the corresponding column (resp. row) of $\tau$ has no non-zero entry. 
%Since we assume $w_\tau$ to be maximal, the entries of $A$ and $B$ are arranged in anti-diagonal fashion.

\begin{example}
	For $\tau=\begin{pmatrix}1&0&0\\0&0&0\\0&1&0\end{pmatrix}$, we have $r=1$, and\[
	w_\tau=\begin{pmatrix}
		0&0&1&2\\
		1&0&0&0\\
		0&0&0&1\\
		0&1&0&0
	\end{pmatrix}.
\]
\end{example}

\subsection{The Steinberg Variety for $\nicefrac GP\times\nicefrac GQ$}
Let $M_\tau$ denote the $B_K$ orbit corresponding to the partial permutation $\tau$, and let $x\in M_\tau$.

%Let $E_1\subset\cdots\subset E_N$ be the standard flag.
We denote by $E_\bullet$ the partial flag $E_n\subset E_{n+1}\subset\cdots\subset E_N$ stabilized by $P$, and by $F_\bullet$ the partial flag $F_1\subset F_2\subset\cdots\subset F_n\subset F_N$ stabilized by $Ad(f(x))Q$.

Let $Z=\mu^{-1}(0)$ be the Steinberg variety of $\nicefrac GP\times\nicefrac GQ$, where $\mu:\nicefrac GP\times\nicefrac GQ\rightarrow\mathcal N_G$ is the moment map.
We write $z\in\mathcal N_G$ as\[
	z=\begin{pmatrix}a&b\\c&d\end{pmatrix}, %\in\mathcal N_G,
\]
with $a,b,c,d$ being $n\times n$ matrices. 
%generic for the property $(P,f(x)Q,z)\in Z_{w_\tau}$.
Suppose $(E_\bullet,F_\bullet,z)\in Z_{w_\tau}$.
We have $z\in\mathfrak u_P$, and $f(x)^{-1}zf(x)\in\mathfrak u_Q$.
It follows from $z\in\u_P$ that $a=c=0$, and that $d$ is strictly upper triangular.
Further, we compute,\begin{align*}
	f(x)^{-1}zf(x)	&=\begin{pmatrix}1&0\\-x&1\end{pmatrix} \begin{pmatrix}0&b\\0&d\end{pmatrix} \begin{pmatrix}1&0\\x&1\end{pmatrix}\\
					&=\begin{pmatrix}-xb&b\\-xd&d\end{pmatrix} \begin{pmatrix}1&0\\x&1\end{pmatrix}\\
					&=\begin{pmatrix}-xb&b\\-xd-xbx&d+bx\end{pmatrix}.
\end{align*}
The condition $f(x)^{-1}zf(x)\in\mathfrak u_Q$ yields that $d+bx=0$, and that $xb$ is strictly upper triangular.
It follows that\begin{align}
\label{shapeOfz}
	z=\begin{pmatrix}0&b\\0&-bx\end{pmatrix},	&&f(x)^{-1}zf(x)=\begin{pmatrix}-xb&b\\0&0\end{pmatrix},
\end{align}
where $b$ is any matrix such that $bx$ and $xb$ are upper triangular.

\subsection{Computing $\Lambda$ from $\tau$.}
Let $x\in M_\tau$ as above, and let $w_\tau$ be the $w$-matrix corresponding to $\tau$, see \cref{partialTow}.
Let $\mathsf T_l$ (resp. $\mathsf T_r$) be the left (resp. right) RSK-tableau of $w_\tau$, and let $\lambda=sh(\mathsf T_r)=sh(\T_l)$.
Following \cref{steinberg}, we see that $Tab(z,E_\bullet)=\mathsf T_l$, and $Tab(z,F_\bullet)=\mathsf T_r$.

Consider $b$ generic in the set $Z_x$, see \cref{ppduality}, and let $z$ be as in \cref{shapeOfz}.
Following \cref{syd}, to compute $\Lambda$, it is sufficient to compute the Jordan types of $z$, $bx$, $xb$, and $\begin{pmatrix} -xb&0\\ x&0\end{pmatrix}$.

We see from \cref{steinberg} that $sh(z)=\lambda$.
Further, we see from \cref{shapeOfz} that the tableau for $xb$ is precisely $\mathsf T_r[n]$.
Next, we compute the tableau for $bx$.
Observe that $e(\mathsf T_l)$ corresponds to the sequence of partitions,\[
	sh(z|\nicefrac{E_N}{E_{N-1}})\leq sh(z|\nicefrac{E_N}{E_{N-2}})\leq\cdots\leq sh(z|\nicefrac{E_N}{E_n})\leq sh(z|E_N).
\]
Hence, $e(\mathsf T_l)[n]$ corresponds to the sequence,\[
	sh(z|\nicefrac{E_N}{E_{N-1}})\leq sh(z|\nicefrac{E_N}{E_{N-2}})\leq\cdots\leq sh(z|\nicefrac{E_N}{E_n}).
\]
Following \cref{shapeOfz}, we see that the above sequence is equivalent to the sequence,\[
	sh(bx|\nicefrac{E_n}{E_{n-1}})\leq sh(bx|\nicefrac{E_n}{E_{n-2}})\leq\cdots\leq sh(bx|E_n).
\]
Consequently, the tableau for $bx$ is precisely $e(e(\mathsf T_l)[n])$.

\subsection{.}
The Jordan type of $\begin{pmatrix}-xb&0\\ x&0\end{pmatrix}$ is $sh(\T'_l)$, where $\T'_l$ is the left tableau of $w_{\tau^\vee}$, the $w$-matrix of the dual of $\tau$.
How do we compute $\tau^\vee$?

\begin{framed}
\subsection{The Fibre over $\mathcal O_\Lambda$}
We can now restate our original problem as follows: 
Given a signed Young diagram $\Lambda$, for what values of $w_\tau$ (equivalently $\tau$) do we have\begin{align}\label{lambdaLR}
	\Lambda_l=\mathsf T_r[n],	&&\Lambda_r=e(e(\mathsf T_l)[n])?
\end{align}

Let $\lambda=sh(\mathsf T_r)=sh(\mathsf T_l)$.
Observe that that $\mathsf T_l$ is uniquely determined by $e(\mathsf T_l)$, which is itself uniquely determined by the standard tableau $e(\mathsf T_l)[n]$, and the partition $\lambda$.
Similarly, $\mathsf T_r$ is uniquely determined by the standard tableau $\mathsf T_r[n]$, and the partition $\lambda$.
Conversely, every pair of row-standard tableau $(\mathsf T_l,\mathsf T_r)$ satisfying $content(\mathsf T_l)=(n,1,\cdots,1)$ and $content(\mathsf T_r)=(1,\cdots,1,n)$ corresponds to a $w_\tau$.

%Recall that the content of $\mathsf T_r$ and $e(\mathsf T_l)$ is $(1,\cdots,1,n)$.
Following \cref{colStrip}, we see that the set of row-standard tableau pairs $(\mathsf T_r,\mathsf T_l)$ satisfying \cref{lambdaLR} is in bijective correspondence with the set of triples\[ 
	\left\{(\mathsf P,\mathsf Q,\lambda)\mid \mathsf P,\mathsf Q\in SYT(n); \lambda\vdash 2n; sh(\lambda\backslash\mathsf P), sh(\lambda\backslash\mathsf Q)\text{ are column strips}\right\},
\]
via the relation $\mathsf T_r[n]=\mathsf P$, $e(\mathsf T_l)[n]=\mathsf Q$, and $\lambda=sh(T_r)=sh(T'_l)$.
%$(\mathsf T_r[n],\mathsf T'_l[n],\lambda)$, where $\mathsf T_r[n]$ and $\mathsf T'_l[n]$ are any pair of standard tableau of size $n$, and $\lambda$ is any partition of $2n$, such that $sh(\lambda\backslash\mathsf T_r[n])$ and $sh(\lambda\backslash\mathsf T'_l[n])$ are column-strips.
\end{framed}


